Can Implicit Bias Explain Generalization? Stochastic Convex Optimization as a Case Study

The notion of implicit bias, or implicit regularization, has been suggested as a means to explain the surprising generalization ability of modern-days overparameterized learning algorithms. This notion refers to the tendency of the optimization algorithm towards a certain structured solution that often generalizes well. Recently, several papers have studied implicit regularization and were able to identify this phenomenon in various scenarios. We revisit this paradigm in arguably the simplest non-trivial setup, and study the implicit bias of Stochastic Gradient Descent (SGD) in the context of Stochastic Convex Optimization. As a first step, we provide a simple construction that rules out the existence of a \emph{distribution-independent} implicit regularizer that governs the generalization ability of SGD. We then demonstrate a learning problem that rules out a very general class of \emph{distribution-dependent} implicit regularizers from explaining generalization, which includes strongly convex regularizers as well as non-degenerate norm-based regularizations. Certain aspects of our constructions point out to significant difficulties in providing a comprehensive explanation of an algorithm's generalization performance by solely arguing about its implicit regularization properties.

==> nips/header_nips.tex <==
%\usepackage[utf8]{inputenc}
\usepackage{algorithm,algorithmic}
% \usepackage{amsfonts}
% \usepackage{amsthm}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}[theorem]
\newcommand{\cM}{\mathbcal{M}}
\newtheorem{lemma}{Lemma}
\newcommand{\cbe}{C_{\textrm{BE}}}
\newcommand{\erf}{\textrm{erf}}
\newcommand{\fullversion}[2]{#1} %Change to #2 in full version.
% \usepackage{amsfonts}
% \usepackage{hyperref}
\newcommand{\cK}{\mathbcal{K}}
\newcommand{\amo}{a.m.o~}
\newcommand{\vectortwo}[2]{\left(\begin{array}{cc} #1 \\ #2\end{array}\right)}
\newtheorem{property}{Property}
%%%%%%%%%%%%%imported
%\newcommand{\wt}[1]{\w^{(#1)}}
\renewcommand{\v}{\mathbf{v}}
\newcommand{\interval}[2]{a_{(#1,#2)}}
\usepackage{framed}
\usepackage{pdfpages}
% \usepackage{lmodern}
\usepackage{caption}
\usepackage{subcaption}
%\usepackage{graphicx}
\usepackage[capitalize]{cleveref}
\usepackage{thm-restate}
\newcommand{\z}{\mathbf{z}}
\newcommand{\cX}{\mathbcal{X}}
%
% ADD PACKAGES here:
%
\newtheorem*{claim*}{Claim}
% \usepackage{amsmath,amsfonts,graphicx}
\newcommand{\f}{\mathbf{f}}
\usepackage{environ}
\usepackage{comment}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cA}{\mathcal{A}}

%
% The following commands set up the lecnum (lecture number)
% counter and make various numbering schemes work relative
% to the lecture number.
%
\newtheorem{exercise}{Exercise}
\newcommand{\ignore}[1]{}
\newcommand{\w}{\mathbf{w}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\expc}{$\alpha-\exp$-concave~}
\newcounter{lecnum}
\newcommand{\lboundary}{\xi_{0}}
\newcommand{\rboundary}{\xi_{1}}
\newcommand{\algref}[1]{Alg. \ref{#1}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\regret}{\mathrm{Regret}_T}
\newcommand{\etwo}{\textbf{e}_2}
\newcommand{\thetatwo}{\theta_2}
\newcommand{\ERM}{F_S}
\newcommand{\vw}{\textbf{v}(\textbf{w})}
\newcommand{\wttwo}{w_2^{(t)}}
\newcommand{\wtone}{w_1^{(t)}}
\newcommand{\eone}{\textbf{e}_1}
\newcommand{\wt}{\textbf{w}^{(t)}}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\renewcommand{\sc}{m^A_\C}
\newcommand{\oput}{{h_S^A}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\vcd}{\mathrm{VC}}
\newcommand{\condition}{some-name-property}
\renewcommand{\u}{\mathbf{u}}
\newcommand{\CP}{\mathbcal{P}}
\newcommand{\gb}{\ell}
\newcommand{\nnabla}{\hat{\nabla}}
\newcommand{\K}{\mathbcal{K}}
\newcommand{\anothersolution}{\psi}
\newcommand{\anothersolone}{\psi_1}
\newcommand{\vsol}{\textbf{v}}
\newcommand{\ftheta}{f_{\theta_1,\theta_2}}
\newcommand{\wone}{\textbf{w}^{(1)}}
\newcommand{\wtwo}{\textbf{w}^{(2)}}

\crefname{property}{property}{properties}
%for proof 3:
\newcommand{\verticalsum}{Y}
\newcommand{\horizontalsum}{X}
\newcommand{\wsone}{w^S_1}
\newcommand{\wstwo}{w_2^S}
\newcommand{\wione}{w_1^{(i)}}
\newcommand{\witwo}{w_2^{(i)}}
\newcommand{\wonetdividedbyten}{w^{(T/10)}_1}
\newcommand{\wtwotdividedbyten}{w^{(T/10)}_2}
\newcommand{\rwonedimension}{u_t}
\newcommand{\ws}{\mathbf{w}_S}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\stoppingtime}{\tau_{2d}}
\newcommand{\ztone}{Z(k)_1}
\newcommand{\zttwo}{Z(k)_2}
\newcommand{\gaussianwithvar}{\phi_2}
\newcommand{\wsnegative}{\Bar{\w}_s}
\newcommand{\Tthreethousand}{\chi}
\newcommand{\squareedge}{\psi}







\newtheorem*{theorem*}{Theorem}
\newtheorem*{lemma*}{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{definition}{Definition}

\newcommand{\rad}{\mathfrak{R}}
%\newtheorem{claim}{Claim}[lecnum]
\newcommand{\dotp}[2]{\langle #1,#2\rangle}
\renewcommand{\L}{\mathbcal{L}}
\newcommand{\zz}{\mathbf{z}}
\renewcommand{\H}{\mathbcal{H}}
\newcommand{\C}{\mathbcal{C}}
\newcommand{\restrict}{\H_{A}}
\newcommand{\gr}{\tau_{\mathbcal{H}}}
\newcommand{\I}{\mathbf{Id}}
% \newcommand{\EE}{\mathop\mathbb{E}}
\newcommand{\EE}{\mathbf{E}}
\renewcommand{\top}{\mathsf{T}}

\DeclareMathOperator*{\argmin}{arg\,min}

% \newcommand{\rl}[1]{\textcolor{red}{rl: #1}}
\newcommand{\tk}[1]{\textcolor{magenta}{\bf tk: #1}}
% \newcommand{\assaf}[1]{\textcolor{blue}{assaf: #1}}
% \newcommand{\mf}[1]{\textcolor{blue}{Meir: #1}}

\newcommand{\wonet}[1]{w_1^{(#1)}}
\newcommand{\wtwot}[1]{w_2^{(#1)}}
\newcommand{\reflect}[1]{\vec{#1}}
\newcommand{\dominating}{$\ell_2$-dominating}
\usepackage{wrapfig}
% \usepackage{microtype}
% \usepackage{graphicx}
%\usepackage{subfigure}
% \usepackage{booktabs} % for professional tables

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2020} with \usepackage[nohyperref]{icml2020} above.
% \usepackage{hyperref}

% Attempt to make hyperref and algorithmic work together better:
%\newcommand{\theHalgorithm}{\arabic{algorithm}}

% Use the following line for the initial blind version submitted for review:

